Human Pose Regression with Residual Log-likelihood Estimation

Heatmap-based methods dominate in the field of human pose estimation by modelling the output distribution through likelihood heatmaps. In contrast, regression-based methods are more efficient but suffer from inferior performance. In this work, we explore maximum likelihood estimation (MLE) to develop an efficient and effective regression-based methods. From the perspective of MLE, adopting different regression losses is making different assumptions about the output density function. A density function closer to the true distribution leads to a better regression performance. In light of this, we propose a novel regression paradigm with Residual Log-likelihood Estimation (RLE) to capture the underlying output distribution. Concretely, RLE learns the change of the distribution instead of the unreferenced underlying distribution to facilitate the training process. With the proposed reparameterization design, our method is compatible with off-the-shelf flow models. The proposed method is effective, efficient and flexible. We show its potential in various human pose estimation tasks with comprehensive experiments. Compared to the conventional regression paradigm, regression with RLE bring 12.4 mAP improvement on MSCOCO without any test-time overhead. Moreover, for the first time, especially on multi-person pose estimation, our regression method is superior to the heatmap-based methods. Our code is available at https://github.com/Jeff-sjtu/res-loglikelihood-regression

==> sections/experiment.tex <==
\section{Experiments}\label{sec:exp}

In this section, we first introduce the datasets employed for quantitative evaluation. Next, ablation experiments are conducted to evaluate the proposed regression paradigm. Finally, we describe how to embed the proposed method into various human pose estimation tasks and compare the quantitative results with state-of-the-art approaches.

\subsection{Datasets}

\paragraph{MPII} MPII~\cite{mpii} is the benchmark dataset for single-person 2D pose estimation. In total, there are about 29k annotated poses for training and 7k for testing. Following previous settings~\cite{integral}, Percentage of Correct Keypoints (PCK) and Area Under Curve (AUC) metrics are used for evaluation.

\paragraph{MSCOCO Keypoint} MSCOCO Keypoint~\cite{mscoco} is a large-scale in-the-wild 2D human pose benchmark dataset. It consists of 150k instances for training and validation. For evaluation, the mean average precision (mAP) over 10 object keypoint similarity (OKS) thresholds is used. The OKS plays the same role as the IoU in object detection.

\paragraph{Human3.6M} Human3.6M~\cite{h36m} is an indoor benchmark for 3D pose estimation. It includes 11 subjects (5 females and 6 males) performing 15 different activities in a laboratory environment. For evaluation, MPJPE and PA-MPJPE are used. Following typical protocols~\cite{integral}, we use 5 subjects (S1, S5, S6, S7, S8) for training and 2 subjects (S9, S11) for evaluation.

\subsection{Ablation Study}
In this study, we evaluate the effectiveness of the proposed regression paradigm. All evaluation is conducted on the MSCOCO validation set as it contains in-the-wild challenging scenes to demonstrate the strength of our method. We adopt ResNet-50 as the network backbone, followed by an average pooling and an FC layer. The FC layer consists of $K \times 3$ neurons, where $K=17$ denotes the number of body keypoints and $3$ for $\mu_x$, $\mu_y$ and $\sigma$. Here, to reduce computation complexity, $\mu_x$ and $\mu_y$ share with a same $\sigma$.

\paragraph{Effect of Residual Likelihood Estimation}

\paragraph{Initial Density}

\paragraph{Flow Model Architecture}

\paragraph{Computation Complexity}

\paragraph{Convergence}

\subsection{Comparison with the State-of-the-art}

==> sections/experiment_new-ablation.tex <==

\section{Experiments on COCO}\label{sec:exp_coco}

We first evaluate the proposed regression paradigm on a large-scale in-the-wild 2D human pose benchmark COCO Keypoint~\cite{mscoco}.
% It consists of 150k instances for training and validation.
% For evaluation, the mean average precision (mAP) over 10 OKS thresholds is used.
% The OKS plays the same role as the IoU in object detection.

\paragraph{Implementation Details.} We embed the proposed regression paradigm into the \textit{top-down} approaches and a \textit{one-stage} approach.

For the \textit{top-down} approach, we adopt a simple architecture consisting of a ResNet~\cite{resnet} backbone, followed by an average pooling layer and an FC layer. The FC layer consists of $K \times 4$ neurons, where $4$ is for $\hat{\boldsymbol{\mu}}$ and $\hat{\boldsymbol{\sigma}}$, and $K=17$ denotes the number of body keypoints. For human detection, we use the person detectors provided by SimplePose~\cite{xiao2018simple} for both the validation set and the test-dev set. Data augmentations and training settings follow previous work~\cite{sun2019deep}. The end-to-end approach, Mask R-CNN~\cite{he2017mask}, is also adopted for ablation study. Implementation is based on Detectron2~\cite{detectron2}. The keypoint head is a stack of $8$ convolutional layers, followed by an average pooling layer and an FC layer. We train for $270,000$ iterations, with a mini-batch of 4 images per GPU and 4 GPUs in total. Other parameters are the same as the original Detectron2.

% The input image is resized to $256 \times 192$. 
% Data augmentation includes random scale ($\pm 25\%$), rotation ($\pm 45^\circ$), flip and random half-body croping following ~\cite{sun2019deep}.
% The learning rate is set to $1 \times 10^{-3}$ at first and reduced by a factor of $10$ at the $170$th and $200$th epoch. We use the Adam solver and train for $230$ epochs, with a mini-batch size of $32$ per GPU and $8$ GPUs in total.
% This model with residual log-likelihood estimation is denoted as \textbf{\textit{SimpleRLE}}.

% \textcolor{red}{[Siyuan add details about Mask R-CNN.]}

% For \textit{one-stage} approach, we adopt the the state-of-the-art method~\cite{wei2020point}. We replace its 2-channel regression head to a 3-channel head for the prediction of both $\hat{\boldsymbol{\mu}}$ and $\hat{\boldsymbol{\sigma}}$. \textcolor{red}{[Wang Can add more details]}.

For the \textit{one-stage} approach, we adopt the state-of-the-art method~\cite{wei2020point}. We replace its 2K-channel regression head with a 4K-channel head for the prediction of both $\hat{\boldsymbol{\mu}}$ and $\hat{\boldsymbol{\sigma}}$. Implementation is based on the official code of \cite{wei2020point}. The other training details are the same as them.

% HRNet-W32 \cite{sun2019deep} is used as our backbone networks.
% Our network is trained with Adam  over 8 GPUs with a mini-batch of 24 images (3 images per GPU).

\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
    \begin{tabular}{c|cc|ccc}
        Method & \# Params & GFLOPs & AP & AP$_{50}$ & AP$_{75}$ \\
        \midrule
        Direct Regression (with $\ell_1$) & {23.6M} & {4.0} & 58.1 & 82.7 & 65.0 \\
        \textbf{Regression with DLE} & {23.6M} & {4.0} & 62.7 & 86.1 & 70.4 \\
        \textbf{Regression with RLE} & {23.6M} & {4.0} & 70.5 & {88.5} & {77.4} \\
        *\textbf{Regression with RLE} & {23.6M} & {4.0} & \textbf{71.3} & \textbf{88.9} & \textbf{78.3} \\
        % \midrule
        % & SimplePose (Heatmap)~\cite{xiao2018simple} & 71.0 & 89.3 & 79.0 \\
        % & Integral Pose~\cite{integral} & 63.0 & 85.6 & 70.0 \\
        % % & \textbf{SimpleRLE ~w/o~ residual log-likelihood} & 62.7 & 86.1 & 70.4 \\
        % % & \textbf{SimpleRLE} & {70.5} & {88.5} & {77.4} \\
        % & \textbf{Regression with RLE}* & \textbf{71.3} & \textbf{88.9} & \textbf{78.3} \\
        % \midrule
        % \multirow{2}{*}{(b)} & HRNet-W32 (Heatmap) & 74.1 & \textbf{90.0} & \textbf{81.5} \\
        % & \textbf{HRNet-W32 + RLE (Regression)} & \textbf{74.3} & 89.7 & 80.8 \\
        % \midrule
        % \multirow{3}{*}{(c)} & Mask R-CNN & 66.0 & \textbf{86.9} & 71.5 \\
        % & \textbf{Mask R-CNN + RLE} & {66.3} & 86.7 & {72.0} \\
        % & \textbf{Mask R-CNN + RLE}* & \textbf{66.7} & 86.7 & \textbf{72.6} \\
        % \midrule
        % \multirow{2}{*}{(d)} & PointSet Anchor (Regression) & 65.2 & 85.3 & 71.1 \\
        % & \textbf{PointSet Anchor + RLE} & \textbf{66.0} & \textbf{85.9} & \textbf{72.1}
    \end{tabular}
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Effect of Residual Log-likelihood Estimation.} The proposed paradigm significantly improves the conventional direct regression with same test-time computational complexity.}\label{tab:rle}
    \vspace{-3mm}
\end{table}


\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
    \begin{tabular}{cc|ccc}
        & Method & AP & AP$_{50}$ & AP$_{75}$ \\
        \midrule
        \multirow{3}{*}{(a)} & SimplePose~\cite{xiao2018simple} & 71.0 & \textbf{89.3} & 79.0 \\
        & Integral Pose~\cite{integral} & 63.0 & 85.6 & 70.0 \\
        % & \textbf{SimpleRLE ~w/o~ residual log-likelihood} & 62.7 & 86.1 & 70.4 \\
        % & \textbf{SimpleRLE} & {70.5} & {88.5} & {77.4} \\
        & *\textbf{Regression with RLE} & \textbf{71.3} & {88.9} & \textbf{79.3} \\
        \midrule
        \multirow{2}{*}{(b)} & HRNet-W32 (Heatmap)~\cite{sun2019deep} & 74.1 & \textbf{90.0} & \textbf{81.5} \\
        & \textbf{HRNet-W32 + RLE (Regression)} & \textbf{74.3} & 89.7 & 80.8 \\
        \midrule
        \multirow{2}{*}{(c)} & Mask R-CNN~\cite{he2017mask} & 66.0 & \textbf{86.9} & 71.5 \\
        % & \textbf{Mask R-CNN + RLE} & {66.3} & 86.7 & {72.0} \\
        & \textbf{Mask R-CNN + RLE} & \textbf{66.7} & 86.7 & \textbf{72.6} \\
        \midrule
        \multirow{2}{*}{(d)} & PointSet Anchor~\cite{wei2020point} & 67.0 & 87.3 & 73.5 \\
        & \textbf{PointSet Anchor + RLE} & \textbf{67.4} & \textbf{87.5} & \textbf{73.9}
    \end{tabular}
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Comparison with the heatmap-based methods.} The proposed paradigm achieves competitive performance to the heatmap-based methods.}\label{tab:heatmap}
\end{table}

\subsection{Ablation Study}\label{sec:ablation}
This section provides ablation experiments on the validation set of COCO. The experiments are mainly conducted with the \textit{top-down} approach with the ResNet-50 backbone.

\paragraph{Effect of Residual Log-likelihood Estimation.}
To study the effectiveness of the proposed regression paradigm, we compare it with the conventional direct regression method. The direct regression model has the same ``Backbone+FC'' architecture, and $\ell_1$ loss is adopted. The experimental results are shown in Tab.~\ref{tab:rle}. As shown, the proposed method brings significant improvement (\textbf{12.4} mAP) to the regression-based method. Then we compare the result with direct likelihood estimation (DLE) to study the effectiveness of residual log-likelihood estimation. The DLE model only adopts the reparameterization strategy and no residual log-likelihood estimation. It is seen that the residual manner provides \textbf{7.8} mAP improvements. Moreover, like previous work~\cite{integral}, we can pre-train the network backbone using heatmap loss. This model achieves the best performance with \textbf{71.3} mAP, which is denoted with $*$.

Note that the flow model does not participate in the inference phase. Therefore, no extra computation is introduced in testing. These experiments demonstrate the superiority of the proposed regression paradigm.

% is also a ResNet-50 backbone followed with an average pooling and an FC layer and $\ell_1$ loss is adopted.
\paragraph{Comparison with the Heatmap-based Methods.}
We further compare our regression method with the heatmap-based methods. As shown in Tab.~\ref{tab:heatmap}(a), our regression method outperforms Integral Pose~\cite{integral} by \textbf{7.5} mAP, and the heatmap supervised SimplePose~\cite{xiao2018simple} by \textbf{0.3} mAP. For the first time, the direct regression method achieves superior performance to the heatmap-based method.

% Comparing to the fully heatmap supervised SimplePose~\cite{xiao2018simple}, our method is only 0.5 mAP lower.

% the backbone network of SimpleRLE can be pre-trained using heatmap loss. We denotes it as SimpleRLE*. In this way, for the first time, the direct regression method surpass the heatmap based SimplePose by \textbf{0.3} mAP.

% Moreover, we also compare with the heatmap-based baseline (\ie SimplePose~\cite{xiao2018simple}) and Integral Pose~\cite{integral}.
% The experimental results are shown in Tab.~\ref{tab:rle}(a). As it shown, the proposed method brings significant improvement to the regression-based method (\textbf{12.4} mAP). Comparing to the Integral Pose~\cite{integral}, which still needs to generate heatmaps, our method brings \textbf{7.5} mAP improvement.

% Besides, we compare the results between residual log-likelihood estimation and direct likelihood estimation. The residual manner provides \textbf{7.8} mAP improvements.

In Tab.~\ref{tab:heatmap}(b), we also implement RLE with HRNet~\cite{sun2019deep} to show our approach is flexible and can be easily embedded into various backbone networks. Since HRNet maintains high resolution throughout the whole process, we adopt soft-argmax to produce coordinates $\hat{\boldsymbol{\mu}}$ and an FC layer to produce $\hat{\boldsymbol{\sigma}}$. It shows that integral with RLE surpasses conventional heatmap by \textbf{0.2} mAP.

Tab.~\ref{tab:heatmap}(c) shows the superiority of RLE on Mask R-CNN, the end-to-end \textit{top-down} approach. Our regression version outperforms the heatmap-based Mask R-CNN by \textbf{0.7} mAP. In Tab.~\ref{tab:heatmap}(d), RLE brings \textbf{0.4} mAP improvement to the state-of-the-art \textit{one-stage} approach. The superiority of RLE is demonstrated in various approaches.

% The superiority of RLE is demonstrated in various approaches. It outperforms the conventional regression paradigm. Further, for the first time, it achieves superior performance to the heatmap-based method.
% This is the first time that the regression-based method achieves competitive performance to the heatmap-based method.

%###########################################################################################
\begin{table*}[t]
    \begin{center}
        % Density
        \begin{minipage}[t]{0.32\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \makeatletter\def\@captype{table}\makeatother
            \begin{tabular}{c|ccc}        
                Distribution & AP & AP$_{50}$ & AP$_{75}$ \\
                \midrule
                Const. Var Gaussian ($\ell_2$) & 36.6 & 70.9 & 33.6 \\
                Const. Var Laplace ($\ell_1$) & 58.1 & 82.7 & 65.0 \\
                Gaussian & 60.2 & 82.9 & 66.6 \\
                Laplace & 67.4 & 86.8 & 74.2 \\
                \midrule
                \textbf{RLE ($Q(\bar{\mathbf{x}}) \sim$ Gaussian)} & 70.0 & 88.1 & 76.7 \\
                \textbf{RLE ($Q(\bar{\mathbf{x}}) \sim$ Laplace)} & \textbf{70.5} & \textbf{88.5} & \textbf{77.4} \\
            \end{tabular}
            }
            \vspace{-2mm}
            \caption{\textbf{Initial Density:} Performance with different hypotheses of the output distribution.}\label{tab:density}
        \end{minipage}
        \quad
        % RealNVP architecture
        \begin{minipage}[t]{0.25\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \makeatletter\def\@captype{table}\makeatother
            \begin{tabular}{c|ccc}        
                ~ & AP & AP$_{50}$ & AP$_{75}$ \\
                \midrule
                $3 \times 64$ & 70.5 & 88.5 & 77.4 \\
                $3 \times 128$ & 70.2 & 88.5 & 77.3 \\
                $3 \times 256$ & 69.6 & 87.9 & 76.5 \\
                $5 \times 32$ & 70.0 & 88.2 & 76.8 \\
                $5 \times 64$ & 70.3 & 88.7 & 77.4 \\
            \end{tabular}
            }
            \vspace{-2mm}
            \caption{\textbf{RealNVP Architecture:} Performance with different architecture of RealNVP.}\label{tab:realnvp}
        \end{minipage}
        \quad
        % Complexity
        \begin{minipage}[t]{0.35\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \makeatletter\def\@captype{table}\makeatother
            \begin{tabular}{c|c}
                Method & Correlation Coefficients \\
                \midrule
                SimplePose (Heatmap) & 0.479 \\
                Regression with Gaussian & 0.476 \\
                Regression with Laplace & 0.522 \\
                \midrule
                \textbf{RLE ($Q(\bar{\mathbf{x}}) \sim$ Gaussian)} & 0.540 \\
                \textbf{RLE ($Q(\bar{\mathbf{x}}) \sim$ Laplace)} & \textbf{0.553} \\
            \end{tabular}
            }
            \vspace{-2mm}
            \caption{\textbf{Correlation testing} on different methods.}
            \label{tab:corr}
\end{minipage}
\end{center}
\vspace{-9mm}
\end{table*}
%###########################################################################################

\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
    \begin{tabular}{l|cccc}
        Method & \#Params & GFLOPs & \tabincell{c}{GFLOPs\\of Net. Head} & AP \\
        \midrule
        % Direct Regression (with $\ell_1$) & \textbf{23.6M} & \textbf{4.0} & 58.1 \\
        \multicolumn{2}{l}{\textit{Heatmap-based}} \\
        Integral Pose~\cite{integral} & 34.0M & 9.7 & 5.7 & 63.4 \\
        SimplePose~\cite{xiao2018simple} & 34.0M & 9.7 & 5.7 & {71.0} \\
        % SimplePose ResNet-152~\cite{xiao2018simple} & 68.6M & 38.2 & \textbf{71.0} \\
        \midrule
        \multicolumn{2}{l}{\textit{Regression-based}} \\
        % \textbf{Regression with RLE} & \textbf{23.6M} & \textbf{4.0} & \textbf{0.0002} & {70.5} \\
        *\textbf{Regression with RLE} & \textbf{23.6M} & \textbf{4.0} & \textbf{0.0002} & \textbf{71.3} \\
        % \textbf{Regression with RLE} ResNet-152 & \textbf{58.3M} & \textbf{25.5} & {70.5}
    \end{tabular}
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Computation complexity and model parameters.}}
    \label{tab:complexity}
    \vspace{-3mm}
\end{table}



\paragraph{Initial Density.} To examine how the assumption of the output distribution affects the regression performance in the context of MLE, we compare the results of different density functions with our method. The Laplace distribution and Gaussian distribution will degenerate to standard $\ell_1$ and $\ell_2$ loss if they are assumed to have constant variances. As shown in Tab.~\ref{tab:density}, the learned distributions of our method provide more than 21.3\% improvements. Different initial densities $Q(\bar{\mathbf{x}})$ for RLE are also tested. There is a large gap between the Gaussian distribution and the Laplace distribution. However, with RLE to learn the change of the density, the difference between these two distributions is significantly reduced. It demonstrates that RLE is robust to different assumptions of the initial density.

% It is seen that the Laplace distribution provide consistent improvements over the Gaussian distribution. \textcolor{red}{[refine]}

\paragraph{RealNVP Architecture.} In Tab.~\ref{tab:realnvp}, we compare different network architecture of the RealNVP~\cite{dinh2016density} model. It shows that the final AP keeps stable with different RealNVP architecture. We argue that learning the residual log-likelihood is easy for the flow model. Thus the results are robust to the change of the architecture.

% \begin{table}[t]
%     \begin{center}
%     \resizebox{\linewidth}{!}
%     {%
%         \begin{tabular}{l|cccc}
%             Model & \#Params & GFLOPs & AP \\
%             \midrule
%             SimplePose~\cite{xiao2018simple} & 34.0 & 12.9 & 70.9 \\
%             Integral~\cite{integral} & & & 63.4\\
%             \midrule
%             SimpleRLE (Ours) & \textbf{23.6} & \textbf{5.4} & \textcolor{red}{70.5}
%         \end{tabular}
%     }
%     \end{center}
%     \caption{\textbf{Computation complexity and model parameters.}}
%     \label{tab:complexity}
% \end{table}

\paragraph{Correlation with Prediction Correctness.}
The estimated standard deviation $\hat{\boldsymbol{\sigma}}$ establishes the correlation with the prediction correctness. The model will a output larger $\hat{\boldsymbol{\sigma}}$ for a more uncertain result. Therefore, $\hat{\boldsymbol{\sigma}}$ plays the same role as the confidence score in the heatmap. We transform the deviation to confidence with Eq.~\ref{eq:conf}. To analysis the correlation of $\hat{\boldsymbol{\sigma}}$ and the prediction correctness, we calculate the Pearson correlation coefficient between the confidence and the OKS to the ground truth on the COCO validation set. The confidence of the heatmap-based prediction~\cite{xiao2018simple} is the maximum value of the heatmap. Tab.~\ref{tab:corr} reveals that RLE has much a stronger correlation to OKS than the heatmap-based method (\textbf{15.2}\% improvement). In real-world applications and other downstream tasks, a reliable confidence score is useful and necessary. RLE address the lack of confidence scores in regression-based methods and provide a more reliable score than the heatmap-based methods.

\paragraph{Computation Complexity.}
The experimental results of computation complexity and model parameters are listed in Tab.~\ref{tab:complexity}. The proposed method achieves comparable results to the heatmap-based methods with significantly lower computation complexity and fewer model parameters. Specifically, the total FLOPs are reduced by \textbf{58.8}\%, and the parameters are reduced by \textbf{30.6}\%. We further calculate the FLOPs of the network head to remove the influence of the network backbone. It shows that the FLOPs of the regression head is only \textbf{1/28500} of the heatmap head, which is almost negligible. The computational superiority of our proposed regression paradigm is of great value in the industry.

% \paragraph{Convergence}

\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
        \begin{tabular}{l|c|ccccc}
            Method & Backbone & AP & AP$_{50}$ & AP$_{75}$ & AP$_{M}$ & AP$_{L}$ \\
            \midrule
            \multicolumn{2}{l}{\textit{Heatmap-based}} \\
            CMU-Pose & 3CM-3PAF & 61.8 & 84.9 & 67.5 & 57.1 & 68.2 \\
            Mask R-CNN~\cite{he2017mask} & ResNet-50 & 63.1 & 87.3 & 68.7 & 57.8 & 71.4 \\
            G-RMI & ResNet-101 & 64.9 & 85.5 & 71.3 & 62.3 & 70.0 \\
            RMPE & PyraNet & 72.3 & 89.2 & 79.1 & 68.0 & 78.6 \\
            AE & Hourglass-4 & 65.5 & 86.8 & 72.3 & 60.6 & 72.6 \\
            PersonLab & ResNet-152 & 68.7 & 89.0 & 75.4 & 64.1 & 75.5\\
            CPN & ResNet-Inception & 72.1 & 91.4 & 80.0 & 68.7 & 77.2 \\
            SimplePose~\cite{xiao2018simple} & ResNet-152 & 73.7 & 91.9 & 81.1 & 70.3 & 80.0\\
            Integral~\cite{integral} & ResNet-101 & 67.8 & 88.2 & 74.8 & 63.9 & 74.0\\
            HRNet~\cite{sun2019deep} & HRNet-W48 & {75.5} & \textbf{92.5} & \textbf{83.3} & {71.9} & \textbf{81.5} \\
            \midrule
            \multicolumn{2}{l}{\textit{Regression-based}} \\
            CenterNet~\cite{zhou2019objects} & Hourglass-2 & 63.0 & 86.8 & 69.6 & 58.9 & 70.4 \\
            SPM & Hourglass-8 & 66.9 & 88.5 & 72.9 & 62.6 & 73.1 \\
            PointSet Anchor~\cite{wei2020point} & HRNet-W48 & 68.7 & 89.9 & 76.3 & 64.8 & 75.3 \\
            \textbf{ResNet + RLE (Ours)} & ResNet-152 & 74.2 & 91.5 & 81.9 & 71.2 & 79.3 \\
            \textbf{*ResNet + RLE (Ours)} & ResNet-152 & 75.1 & 91.8 & 82.8 & 72.0 & 80.2 \\
            \textbf{HRNet + RLE (Ours)} & HRNet-W48 & \textbf{75.7} & {92.3} & {82.9} & \textbf{72.3} & {81.3} \\
        \end{tabular}
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Results on COCO test-dev} compared to the state-of-the-art methods.}
    \label{tab:coco_main}
    \vspace{-3mm}
\end{table}

\subsection{Compare with the State-of-the-art}
In this experiment, we compare the proposed RLE with the state-of-the-art methods on COCO test-dev. Quantitative results are reported in Tab.~\ref{tab:coco_main}. The proposed regression paradigm significantly outperforms other regression-based methods by \textbf{7.0} mAP and achieves state-of-the-art performance. Compared to the same backbone heatmap-based methods, our regression method is \textbf{1.4} mAP higher with ResNet-152 and \textbf{0.2} mAP higher with HRNet-W48. We demonstrate that heatmap is not the only solution to human pose estimation. Regression-based methods have great potential and can achieve superior performance than heatmap-based methods.

% \begin{figure}[t]
%     \begin{center}
%     \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%     %\includegraphics[width=0.8\linewidth]{egfigure.eps}
%     \end{center}
%     \caption{\textbf{Convergence curve.}}
%     \label{fig:convergence}
% \end{figure}

% \begin{table}[t]
%     \begin{center}
%     \resizebox{\linewidth}{!}
%     {%
%         \begin{tabular}{l|ccccccc|c}
%             Method & Hea & Sho & Elb & Wri & Hip & Kne & Ank & Total \\
%             \midrule
%             \textit{heatmap-Based} \\
%             Insafutdinov \etal~\cite{} & 96.8 & 95.2 & 89.3 & 84.4 & 88.4 & 83.4 & 78.0 & 88.5 \\
%             Wei \etal~\cite{} & 97.8 & 95.0 & 88.7 & 84.0 & 88.4 & 82.8 & 79.4 & 88.5 \\
%             Bulat \etal~\cite{} & 97.9 & 95.1 & 89.9 & 85.3 & 89.4 & 85.7 & 81.7 & 89.7 \\
%             Newell \etal~\cite{} & 98.2 & 96.3 & 91.2 & 87.1 & 90.1 & 87.4 & 83.6 & 90.9 \\
%             Sun \etal~\cite{}  & 98.1 & 96.2 & 91.2 & 87.2 & 89.8 & 87.4 & 84.1 & 91.0 \\
%             Tang \etal~\cite{}  & 97.4 & 96.4 & 92.1 & 87.7 & 90.2 & 87.7 & 84.3 & 91.2 \\
%             Ning \etal~\cite{}  & 98.1 & 96.3 & 92.2 & 87.8 & 90.6 & 87.6 & 82.7 & 91.2 \\
%             Luvizon \etal~\cite{} & 98.1 & 96.6 & 92.0 & 87.5 & 90.6 & 88.0 & 82.7 & 91.2 \\
%             Chu \etal~\cite{} & 98.5 & 96.3 & 91.9 & 88.1 & 90.6 & 88.0 & 85.0 & 91.5 \\
%             Chou \etal~\cite{} & 98.2 & 96.8 & 92.2 & 88.0 & 91.3 & 89.1 & 84.9 & 91.8 \\
%             Chen \etal~\cite{} & 98.1 & 96.5 & 92.5 & 88.5 & 90.2 & \textbf{89.6} & 86.0 & 91.9 \\
%             Yang \etal~\cite{} & 98.5 & 96.7 & 92.5 & 88.7 & 91.1 & 88.6 & 86.0 & 92.0 \\  
%             Ke \etal~\cite{} & 98.5 & 96.8 & 92.7 & 88.4 & 90.6 & 89.3 & \textbf{86.3} & 92.1 \\  
%             Tang \etal~\cite{} & 98.4 & \textbf{96.9} & 92.6 & 88.7 & \textbf{91.8} & 89.4 & 86.2 & \textbf{92.3} \\ 
%             SimpleBaseline~\cite{}& 98.5 & 96.6 & 91.9 & 87.6 & 91.1 & 88.1 & 84.1 & 91.5 \\
%             HRNet-W32~\cite{} &\textbf{98.6}  & \textbf{96.9}  & \textbf{92.8}  & \textbf{89.0}  & 91.5  & 89.0 & 85.7 & \textbf{92.3} \\
%             \midrule
%             \textit{Regression Based} \\
%             Carreira \etal~\cite{} \\
%             Sun \etal~\cite{} \\
%             Integral~\cite{integral} \\
%             \textbf{SimpleRLE (ResNet-50)} \\
%             \textbf{SimpleRLE (HRNet-W32)}
%         \end{tabular}
%     }
%     \end{center}
%     \caption{\textbf{Results on MPII test set (PCKh@0.5).}}
%     \label{tab:mpii_main}
% \end{table}


\section{Experiments on MPII}\label{sec:exp_mpii}

In multi-person pose estimation, the final mAP is affected by both the location accuracy and the confidence score. To study how RLE affect the location accuracy and eliminate the impact of the confidence score, we evaluate the proposed regression paradigm on the MPII~\cite{mpii} dataset. Following previous settings~\cite{integral}, PCK and AUC are used for evaluation. We adopt the same ResNet-50 + FC model for single-person 2D pose estimation. Data augmentations and training settings are similar to the experiments on COCO.
% MPII is the benchmark dataset for single-person 2D pose estimation. In total, there are about 29k annotated poses for training and 7k for testing.
% \paragraph{Implementation Details}
% The input image is resized to $256 \times 192$. Data augmentation includes random scale ($\pm 25\%$), rotation ($\pm 45^\circ$), flip and random half-body croping. The learning rate is set to $1 \times 10^{-3}$ at first and reduced by a factor of $10$ at the $170$th and $200$th epoch. We use the Adam solver and train for $210$ epochs, with a mini-batch size of $32$ per GPU and $8$ GPUs in total.
%The testing procedure is almost the same to that in COCO except that we adopt the standard testing strategy to use the provided person boxes instead of detected person boxes. Following ~\cite{}, a six-scale pyramid testing procedure is performed.

\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
        \begin{tabular}{c|ccc}
            Method & PCKh@0.5 & PCKh@0.1 & AUC \\
            \midrule
            Direct Regression & 83.8 & 23.6 & 52.6 \\
            SimplePose (Heatmap)~\cite{xiao2018simple} & \textbf{87.1} & {25.4} & \textbf{56.2} \\
            % Integral Pose~\cite{integral} & 86.5 & 31.0 & 57.8 \\
            \midrule
            \textbf{Regression with RLE} & 85.5 & {26.7} & 55.1 \\
            *\textbf{Regression with RLE} & 85.8 & \textbf{27.1} & 55.5 \\
            % \textbf{Integral + RLE} & 86.9 & \textbf{33.3} & \textbf{59.0}
        \end{tabular}
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Effect of Residual Log-likelihood Estimation on MPII validation set.}}
    \label{tab:ablation_mpii}
    \vspace{-3mm}
\end{table}

\paragraph{Ablation Study.}
Tab.~\ref{tab:ablation_mpii} shows the comparison among methods using heatmaps, direct regression and RLE. RLE surpasses the direct regression baseline. While MPII is less challenging than COCO, the improvement is still significant on PCKh@0.1 (\textbf{13.1}\%) with high localization accuracy requirement. Compared to the heatmap-based method, RLE achieves comparable performance (5.1\% PCKh@0.1 higher, 1.8\% PCKh@0.5 lower and 1.9\% AUC lower), and the pre-trained model achieves the best PCKh@0.1 results. RLE shows the superiority in high precision localization.
% Besides, the combination of integral regression and RLE shows the most accurate localization ability. It outperforms the heatmap based method on PCKh@0.1 by \textbf{10.3}\%, revealing the effectiveness and flexibility of our proposed regression paradigm.
% Tab.~\ref{tab:ablation_mpii} shows the PCKh@0.5 results. We implementation the SimpleRLE model with two model backbone, ResNet-50 and HRNet-W32. Our models are trained on MPII data, no extra data is added. It is shown that the proposed method outperform other regression-based methods and achieves competitive results with the heatmap-based methods. \textcolor{red}{[more]}


%###########################################################################################
% \begin{table*}[t]
%     \begin{center}
%         \begin{minipage}[t]{0.49\textwidth}
%             \centering
%             \resizebox{\linewidth}{!}
%             {%
%             \begin{tabular}{l|cccccc|c}
%                 Method & \tabincell{c}{Zhou \\ \cite{}} & \tabincell{c}{Martinez \\ \cite{}} & \tabincell{c}{Fang \\ \cite{}} & \tabincell{c}{Sun \\ \cite{}} & \tabincell{c}{Sun \\ \cite{}} & \tabincell{c}{Moon \\ \cite{}} & SimpleRLE (Ours) \\
%                     \midrule
%                     MPJPE & & & & & & & \textbf{48.8}
%                 \end{tabular}
%             }
%             \caption{\textbf{Results on Human3.6M.} (Single-stage)}
%             \label{tab:h36m_single_main}
%         \end{minipage}
%         ~
%         \begin{minipage}[t]{0.49\textwidth}
%             \centering
%             \resizebox{\linewidth}{!}
%             {%
%                 \begin{tabular}{l|cccccc|c}
%                     Method & \tabincell{c}{Zhou \\ \cite{}} & \tabincell{c}{Martinez \\ \cite{}} & \tabincell{c}{Fang \\ \cite{}} & \tabincell{c}{Sun \\ \cite{}} & \tabincell{c}{Sun \\ \cite{}} & \tabincell{c}{SRNet \\ \cite{}} & SRNet + RLE (Ours) \\
%                     \midrule
%                     MPJPE
%                 \end{tabular}
%             }
%             \caption{\textbf{Results on Human3.6M.} (Two-stage)}
%             \label{tab:h36m_two_main}
%         \end{minipage}
%     \end{center}
% \end{table*}
%###########################################################################################


\section{Experiments on Human3.6M}\label{sec:exp_h36m}

Human3.6M~\cite{h36m} is an indoor benchmark for 3D pose estimation. For evaluation, MPJPE and PA-MPJPE are used. Following typical protocols~\cite{integral}, we use (S1, S5, S6, S7, S8) for training and (S9, S11) for evaluation.
% It includes 11 subjects (5 females and 6 males) performing 15 different activities in a laboratory environment

\paragraph{Implementation Details.}
% There are two types of approaches to the problem of single-person 3D pose estimation: \textit{single-stage} and \textit{two-stage}.
% The FC layer consists of $K \times 4$ neurons.

For the \textit{single-stage} approach, we adopt the same ResNet-50 + FC architecture. The input image is resized to $256 \times 256$. Data augmentation includes random scale ($\pm 30\%$), rotation ($\pm 30^\circ$), color ($\pm 20\%$) and flip. The learning rate is set to $1 \times 10^{-3}$ at first and reduced by a factor of $10$ at the $90$th and $120$ epoch. We use the Adam solver and train for $140$ epochs, with a mini-batch size of $32$ per GPU and $8$ GPUs in total. The 2D and 3D mixed data training strategy (MPII + Human3.6M) is applied. The testing procedure is the same as the previous works~\cite{integral}.

For the \textit{two-stage} approach, we embed the proposed regression paradigm into the classic baseline~\cite{martinez2017simple} and the state-of-the-art model~\cite{zeng2020srnet}. 2D ground-truth poses are taken as inputs. For data normalization, we follow previous works~\cite{zeng2020srnet,pavllo2019videopose3d,zhaoCVPR19semantic}. Horizontal flip is used during training and inference. The initial learning rate is $1 \times 10^{-3}$ and decays $5\%$ after each epoch. We use the Adam solver and train for $80$ epochs, with a mini-batch size of $1024$.
% to normalize 2d pose into $[-1,1]$ according to the width and height of images, and normalize 3d pose under camera coordinate system to a relative coordinate, which takes the root keypoint as the origin.
% For model structure, we compare six-layer structure with other methods. Each layer, except the output layer, is consist of batch normalization, LeakyReLU. And every two layers are connected by a residual connection. The dimension of hidden layers is $1024$.
% For data augmentation, like ~\cite{pavllo2019videopose3d,zeng2020srnet}, we use horizontal flip during training and inference stages.
% Furthermore, we also use Adam as the optimizer and train $80$ epochs from scratch. The batch size is $1024$.



\paragraph{Ablation Study.} In Tab.~\ref{tab:ablation_h36m}, we report the performance comparison between RLE and the baselines on both \textit{single-stage} and \textit{two-stage} approaches. It is seen that RLE reduces the error of \textit{single-stage} regression baseline by \textbf{1.5} mm and the heatmap-based Integral Pose~\cite{integral} by \textbf{0.6} mm. Besides, without 3D heatmaps, our regression method significantly reduces the FLOPs by \textbf{61.7}\% and the model parameters by \textbf{30.6}\%. For the \textit{two-stage} approach, RLE brings \textbf{2.7} mm improvement to the regression baseline without any test-time overhead.

\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
        \begin{tabular}{l|cc|cc}
            Method & \#Params & GFLOPs & MPJPE~$\downarrow$ & PA-MPJPE~$\downarrow$ \\
            \midrule
            \multicolumn{2}{l}{\textit{Single-stage}} \\
            Direct Regression & 23.8M & 5.4 & 50.1 & 39.3 \\
            Integral Pose~\cite{integral} & 34.3M & 14.1 & 49.2 & 39.1 \\
            \textbf{Regression with RLE} & \textbf{23.8M} & \textbf{5.4} & \textbf{48.6} & \textbf{38.5} \\
            % \textbf{Integral + SimpleRLE} & & {48.9} \\
            \midrule
            \multicolumn{2}{l}{\textit{Two-stage}} \\
            FC Baseline & 4.3M & 0.275 & 43.6 & 33.2 \\
            \textbf{FC Baseline + RLE} & 4.3M & 0.275 & \textbf{40.9} & \textbf{31.1}
        \end{tabular}
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Ablation study on Human3.6M.}}
    \label{tab:ablation_h36m}
    \vspace{-1mm}
\end{table}

\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
    \begin{tabular}{l|ccccc|c}
        Method &\tabincell{c}{Sun \\ \cite{sun2017compositional}} & \tabincell{c}{Nibali \\ \cite{nibali20193d}} &  \tabincell{c}{Sun \\ \cite{integral}} & \tabincell{c}{Moon \\ \cite{moon}} & \tabincell{c}{Zhou \\ \cite{zhou2019hemlets}} & Ours \\
            \midrule
            \#Params & - & 57.9M & 34.3M & 34.3M & 49.6M & \textbf{23.8}M \\
            GFLOPs & - & 29.3 & 14.1 & 14.1 & 41.4 & \textbf{5.4} \\
            MPJPE & 59.1 & 49.5 & 49.6 & 53.3 & \textbf{47.7} & 48.6
        \end{tabular}
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Single-stage Results on Human3.6M.}}
    \label{tab:h36m_single_main}
    \vspace{-1mm}
\end{table}

\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
    % \setlength{\tabcolsep}{1mm}{
        \begin{tabular}{l|cccccc|c}
            % Method  & \tabincell{c}{Pose2Mesh \\ \cite{choi2020pose2mesh}} &\tabincell{c}{FC Baseline \\ \cite{martinez2017simple}} & \tabincell{c}{SemGCN \\ \cite{zhaoCVPR19semantic}} & \tabincell{c}{SemGCN \\w/PG \cite{fang2018learning}} & \tabincell{c}{Pre-agg GCN\\ \cite{liu2020comprehensive}} & \tabincell{c}{SRNet \\ \cite{zeng2020srnet}} & \tabincell{c}{SRNet + RLE \\ (Ours)} \\
            Method  & \tabincell{c}{Choi \\ \cite{choi2020pose2mesh}} &\tabincell{c}{Martinez \\ \cite{martinez2017simple}} & \tabincell{c}{Zhao \\ \cite{zhaoCVPR19semantic}} & \tabincell{c}{Fang \\ \cite{fang2018learning}} & \tabincell{c}{Liu\\ \cite{liu2020comprehensive}} & \tabincell{c}{Zeng \\ \cite{zeng2020srnet}} & \tabincell{c}{Ours} \\
            \midrule
            MPJPE & 55.5 & 45.5 & 43.8 & 42.5 & 37.8 & 36.5 & \textbf{36.3} \\
        \end{tabular}
    % }
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Two-stage Results on Human3.6M.} Our result is based on SRNet~\cite{zeng2020srnet} with RLE.}
    \label{tab:h36m_two_main}
    \vspace{-3mm}
\end{table}

\paragraph{Compare the the State-of-the-art.}
In this experiment, we compare the proposed regression paradigm with both \textit{single-stage} and \textit{two-stage} state-of-the-art methods in Tab.~\ref{tab:h36m_single_main} and Tab.~\ref{tab:h36m_two_main}. For \textit{single-stage}, our method achieves comparable performance to the state-of-the-art methods while reducing the FLOPs by \textbf{86.7}\%. The model parameters and FLOPs are calculated using the official code of these methods. Note that \cite{zhou2019hemlets} only releases the testing code. For fare comparison, we re-train the model with the same training settings as ours. For \textit{two-stage}, our method is based on SRNet~\cite{zeng2020srnet} with RLE. It achieves state-of-the-art performance by 0.2 mm improvement to the original SRNet.

==> sections/experiment_new-main-results.tex <==

\section{Experiments on COCO}\label{sec:exp_coco}

We first evaluate the proposed regression paradigm on a large-scale in-the-wild 2D human pose benchmark COCO Keypoint~\cite{mscoco}.
% It consists of 150k instances for training and validation.
% For evaluation, the mean average precision (mAP) over 10 OKS thresholds is used.
% The OKS plays the same role as the IoU in object detection.

\paragraph{Implementation Details.} We embed the proposed regression paradigm into the \textit{top-down} approaches and a \textit{one-stage} approach.

For the \textit{top-down} approach, we adopt a simple architecture consisting of a ResNet~\cite{resnet} backbone, followed by an average pooling layer and an FC layer. The FC layer consists of $K \times 4$ neurons, where $4$ is for $\hat{\boldsymbol{\mu}}$ and $\hat{\boldsymbol{\sigma}}$, and $K=17$ denotes the number of body keypoints. For human detection, we use the person detectors provided by SimplePose~\cite{xiao2018simple} for both the validation set and the test-dev set. Data augmentations and training settings follow previous work~\cite{sun2019deep}. The end-to-end approach, Mask R-CNN~\cite{he2017mask}, is also adopted for ablation study. Implementation is based on Detectron2~\cite{detectron2}. The keypoint head is a stack of $8$ convolutional layers, followed by an average pooling layer and an FC layer. We train for $270,000$ iterations, with a mini-batch of 4 images per GPU and 4 GPUs in total. Other parameters are the same as the original Detectron2.

% The input image is resized to $256 \times 192$. 
% Data augmentation includes random scale ($\pm 25\%$), rotation ($\pm 45^\circ$), flip and random half-body croping following ~\cite{sun2019deep}.
% The learning rate is set to $1 \times 10^{-3}$ at first and reduced by a factor of $10$ at the $170$th and $200$th epoch. We use the Adam solver and train for $230$ epochs, with a mini-batch size of $32$ per GPU and $8$ GPUs in total.
% This model with residual log-likelihood estimation is denoted as \textbf{\textit{SimpleRLE}}.

% \textcolor{red}{[Siyuan add details about Mask R-CNN.]}

% For \textit{one-stage} approach, we adopt the the state-of-the-art method~\cite{wei2020point}. We replace its 2-channel regression head to a 3-channel head for the prediction of both $\hat{\boldsymbol{\mu}}$ and $\hat{\boldsymbol{\sigma}}$. \textcolor{red}{[Wang Can add more details]}.

For the \textit{one-stage} approach, we adopt the state-of-the-art method~\cite{wei2020point}. We replace its 2K-channel regression head with a 4K-channel head for the prediction of both $\hat{\boldsymbol{\mu}}$ and $\hat{\boldsymbol{\sigma}}$. Implementation is based on the official code of \cite{wei2020point}. The other training details are the same as them.

% HRNet-W32 \cite{sun2019deep} is used as our backbone networks.
% Our network is trained with Adam  over 8 GPUs with a mini-batch of 24 images (3 images per GPU).

\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
    \begin{tabular}{c|cc|ccc}
        Method & \# Params & GFLOPs & AP & AP$_{50}$ & AP$_{75}$ \\
        \midrule
        Direct Regression (with $\ell_1$) & {23.6M} & {4.0} & 58.1 & 82.7 & 65.0 \\
        \textbf{Regression with DLE} & {23.6M} & {4.0} & 62.7 & 86.1 & 70.4 \\
        \textbf{Regression with RLE} & {23.6M} & {4.0} & 70.5 & {88.5} & {77.4} \\
        *\textbf{Regression with RLE} & {23.6M} & {4.0} & \textbf{71.3} & \textbf{88.9} & \textbf{78.3} \\
        % \midrule
        % & SimplePose (Heatmap)~\cite{xiao2018simple} & 71.0 & 89.3 & 79.0 \\
        % & Integral Pose~\cite{integral} & 63.0 & 85.6 & 70.0 \\
        % % & \textbf{SimpleRLE ~w/o~ residual log-likelihood} & 62.7 & 86.1 & 70.4 \\
        % % & \textbf{SimpleRLE} & {70.5} & {88.5} & {77.4} \\
        % & \textbf{Regression with RLE}* & \textbf{71.3} & \textbf{88.9} & \textbf{78.3} \\
        % \midrule
        % \multirow{2}{*}{(b)} & HRNet-W32 (Heatmap) & 74.1 & \textbf{90.0} & \textbf{81.5} \\
        % & \textbf{HRNet-W32 + RLE (Regression)} & \textbf{74.3} & 89.7 & 80.8 \\
        % \midrule
        % \multirow{3}{*}{(c)} & Mask R-CNN & 66.0 & \textbf{86.9} & 71.5 \\
        % & \textbf{Mask R-CNN + RLE} & {66.3} & 86.7 & {72.0} \\
        % & \textbf{Mask R-CNN + RLE}* & \textbf{66.7} & 86.7 & \textbf{72.6} \\
        % \midrule
        % \multirow{2}{*}{(d)} & PointSet Anchor (Regression) & 65.2 & 85.3 & 71.1 \\
        % & \textbf{PointSet Anchor + RLE} & \textbf{66.0} & \textbf{85.9} & \textbf{72.1}
    \end{tabular}
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Effect of Residual Log-likelihood Estimation.} The proposed paradigm significantly improves the conventional direct regression with same test-time computational complexity.}\label{tab:rle}
    \vspace{-3mm}
\end{table}


\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
    \begin{tabular}{cc|ccc}
        & Method & AP & AP$_{50}$ & AP$_{75}$ \\
        \midrule
        \multirow{3}{*}{(a)} & SimplePose~\cite{xiao2018simple} & 71.0 & \textbf{89.3} & 79.0 \\
        & Integral Pose~\cite{integral} & 63.0 & 85.6 & 70.0 \\
        % & \textbf{SimpleRLE ~w/o~ residual log-likelihood} & 62.7 & 86.1 & 70.4 \\
        % & \textbf{SimpleRLE} & {70.5} & {88.5} & {77.4} \\
        & *\textbf{Regression with RLE} & \textbf{71.3} & {88.9} & \textbf{79.3} \\
        \midrule
        \multirow{2}{*}{(b)} & HRNet-W32 (Heatmap)~\cite{sun2019deep} & 74.1 & \textbf{90.0} & \textbf{81.5} \\
        & \textbf{HRNet-W32 + RLE (Regression)} & \textbf{74.3} & 89.7 & 80.8 \\
        \midrule
        \multirow{2}{*}{(c)} & Mask R-CNN~\cite{he2017mask} & 66.0 & \textbf{86.9} & 71.5 \\
        % & \textbf{Mask R-CNN + RLE} & {66.3} & 86.7 & {72.0} \\
        & \textbf{Mask R-CNN + RLE} & \textbf{66.7} & 86.7 & \textbf{72.6} \\
        \midrule
        \multirow{2}{*}{(d)} & PointSet Anchor~\cite{wei2020point} & 67.0 & 87.3 & 73.5 \\
        & \textbf{PointSet Anchor + RLE} & \textbf{67.4} & \textbf{87.5} & \textbf{73.9}
    \end{tabular}
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Comparison with the heatmap-based methods} on COCO validation set. The proposed paradigm achieves competitive performance to the heatmap-based methods.}\label{tab:heatmap}
\end{table}

\subsection{Main Results}\label{sec:main_exp}
% In this section, we study the efficacy of RLE by comprehensive experiments.
% we compare RLE with conventional regression methods and heatmap-based methods

% \subsection{Ablation Study}\label{sec:ablation}
% This section provides ablation experiments on the validation set of COCO. The experiments are mainly conducted with the \textit{top-down} approach with the ResNet-50 backbone.

\paragraph{Effect of Residual Log-likelihood Estimation.}
To study the effectiveness of the proposed regression paradigm, we compare it with the conventional direct regression method. The direct regression model has the same ``Backbone+FC'' architecture, and $\ell_1$ loss is adopted. The experimental results on COCO validation set are shown in Tab.~\ref{tab:rle}. As shown, the proposed method brings significant improvement (\textbf{12.4} mAP) to the regression-based method. Then we compare the result with direct likelihood estimation (DLE) to study the effectiveness of residual log-likelihood estimation. The DLE model only adopts the reparameterization strategy and no residual log-likelihood estimation. It is seen that the residual manner provides \textbf{7.8} mAP improvements. Moreover, like previous work~\cite{integral}, we can pre-train the network backbone using heatmap loss. This model achieves the best performance with \textbf{71.3} mAP, which is denoted with $*$.

Note that the flow model does not participate in the inference phase. Therefore, no extra computation is introduced in testing. These experiments demonstrate the superiority of the proposed regression paradigm.

% is also a ResNet-50 backbone followed with an average pooling and an FC layer and $\ell_1$ loss is adopted.
\paragraph{Comparison with the Heatmap-based Methods.}
We further compare our regression method with the heatmap-based methods. As shown in Tab.~\ref{tab:heatmap}(a), our regression method outperforms Integral Pose~\cite{integral} by \textbf{7.5} mAP, and the heatmap supervised SimplePose~\cite{xiao2018simple} by \textbf{0.3} mAP. For the first time, the direct regression method achieves superior performance to the heatmap-based method.

% Comparing to the fully heatmap supervised SimplePose~\cite{xiao2018simple}, our method is only 0.5 mAP lower.

% the backbone network of SimpleRLE can be pre-trained using heatmap loss. We denotes it as SimpleRLE*. In this way, for the first time, the direct regression method surpass the heatmap based SimplePose by \textbf{0.3} mAP.

% Moreover, we also compare with the heatmap-based baseline (\ie SimplePose~\cite{xiao2018simple}) and Integral Pose~\cite{integral}.
% The experimental results are shown in Tab.~\ref{tab:rle}(a). As it shown, the proposed method brings significant improvement to the regression-based method (\textbf{12.4} mAP). Comparing to the Integral Pose~\cite{integral}, which still needs to generate heatmaps, our method brings \textbf{7.5} mAP improvement.

% Besides, we compare the results between residual log-likelihood estimation and direct likelihood estimation. The residual manner provides \textbf{7.8} mAP improvements.

In Tab.~\ref{tab:heatmap}(b), we also implement RLE with HRNet~\cite{sun2019deep} to show our approach is flexible and can be easily embedded into various backbone networks. Since HRNet maintains high resolution throughout the whole process, we adopt soft-argmax to produce coordinates $\hat{\boldsymbol{\mu}}$ and an FC layer to produce $\hat{\boldsymbol{\sigma}}$. It shows that integral with RLE surpasses conventional heatmap by \textbf{0.2} mAP.

Tab.~\ref{tab:heatmap}(c) shows the superiority of RLE on Mask R-CNN, the end-to-end \textit{top-down} approach. Our regression version outperforms the heatmap-based Mask R-CNN by \textbf{0.7} mAP. In Tab.~\ref{tab:heatmap}(d), RLE brings \textbf{0.4} mAP improvement to the state-of-the-art \textit{one-stage} approach. The superiority of RLE is demonstrated in various approaches.

% The superiority of RLE is demonstrated in various approaches. It outperforms the conventional regression paradigm. Further, for the first time, it achieves superior performance to the heatmap-based method.
% This is the first time that the regression-based method achieves competitive performance to the heatmap-based method.

\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
        \begin{tabular}{l|c|ccccc}
            Method & Backbone & AP & AP$_{50}$ & AP$_{75}$ & AP$_{M}$ & AP$_{L}$ \\
            \midrule
            \multicolumn{2}{l}{\textit{Heatmap-based}} \\
            CMU-Pose & 3CM-3PAF & 61.8 & 84.9 & 67.5 & 57.1 & 68.2 \\
            Mask R-CNN~\cite{he2017mask} & ResNet-50 & 63.1 & 87.3 & 68.7 & 57.8 & 71.4 \\
            G-RMI & ResNet-101 & 64.9 & 85.5 & 71.3 & 62.3 & 70.0 \\
            RMPE & PyraNet & 72.3 & 89.2 & 79.1 & 68.0 & 78.6 \\
            AE & Hourglass-4 & 65.5 & 86.8 & 72.3 & 60.6 & 72.6 \\
            PersonLab & ResNet-152 & 68.7 & 89.0 & 75.4 & 64.1 & 75.5\\
            CPN & ResNet-Inception & 72.1 & 91.4 & 80.0 & 68.7 & 77.2 \\
            SimplePose~\cite{xiao2018simple} & ResNet-152 & 73.7 & 91.9 & 81.1 & 70.3 & 80.0\\
            Integral~\cite{integral} & ResNet-101 & 67.8 & 88.2 & 74.8 & 63.9 & 74.0\\
            HRNet~\cite{sun2019deep} & HRNet-W48 & {75.5} & \textbf{92.5} & \textbf{83.3} & {71.9} & \textbf{81.5} \\
            \midrule
            \multicolumn{2}{l}{\textit{Regression-based}} \\
            CenterNet~\cite{zhou2019objects} & Hourglass-2 & 63.0 & 86.8 & 69.6 & 58.9 & 70.4 \\
            SPM & Hourglass-8 & 66.9 & 88.5 & 72.9 & 62.6 & 73.1 \\
            PointSet Anchor~\cite{wei2020point} & HRNet-W48 & 68.7 & 89.9 & 76.3 & 64.8 & 75.3 \\
            \textbf{ResNet + RLE (Ours)} & ResNet-152 & 74.2 & 91.5 & 81.9 & 71.2 & 79.3 \\
            \textbf{*ResNet + RLE (Ours)} & ResNet-152 & 75.1 & 91.8 & 82.8 & 72.0 & 80.2 \\
            \textbf{HRNet + RLE (Ours)} & HRNet-W48 & \textbf{75.7} & {92.3} & {82.9} & \textbf{72.3} & {81.3} \\
        \end{tabular}
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Results on COCO test-dev} compared to the state-of-the-art methods.}
    \label{tab:coco_main}
    \vspace{-3mm}
\end{table}

%###########################################################################################
\begin{table*}[t]
    \begin{center}
        % Complexity
        \begin{minipage}[t]{0.3\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \makeatletter\def\@captype{table}\makeatother
            \begin{tabular}{c|c}
                Method & Correlation \\
                \midrule
                SimplePose (Heatmap) & 0.479 \\
                Regression with Gaussian & 0.476 \\
                Regression with Laplace & 0.522 \\
                \midrule
                \textbf{RLE ($Q(\bar{\mathbf{x}}) \sim$ Gaussian)} & 0.540 \\
                \textbf{RLE ($Q(\bar{\mathbf{x}}) \sim$ Laplace)} & \textbf{0.553} \\
            \end{tabular}
            }
            \vspace{-2mm}
            \caption{\textbf{Correlation testing} on different methods.}
            \label{tab:corr}
        \end{minipage}
        \quad
        % Density
        \begin{minipage}[t]{0.4\textwidth}
        \centering
            \resizebox{\linewidth}{!}
            {%
            \setlength{\tabcolsep}{1mm}{
            \begin{tabular}{l|cccc}
                Method & \#Params & GFLOPs & \tabincell{c}{GFLOPs\\of Net. Head} & AP \\
                \midrule
                % Direct Regression (with $\ell_1$) & \textbf{23.6M} & \textbf{4.0} & 58.1 \\
                \multicolumn{2}{l}{\textit{Heatmap-based}} \\
                Integral Pose~\cite{integral} & 34.0M & 9.7 & 5.7 & 63.4 \\
                SimplePose~\cite{xiao2018simple} & 34.0M & 9.7 & 5.7 & {71.0} \\
                % SimplePose ResNet-152~\cite{xiao2018simple} & 68.6M & 38.2 & \textbf{71.0} \\
                \midrule
                \multicolumn{2}{l}{\textit{Regression-based}} \\
                % \textbf{Regression with RLE} & \textbf{23.6M} & \textbf{4.0} & \textbf{0.0002} & {70.5} \\
                *\textbf{Regression with RLE} & \textbf{23.6M} & \textbf{4.0} & \textbf{0.0002} & \textbf{71.3} \\
                % \textbf{Regression with RLE} ResNet-152 & \textbf{58.3M} & \textbf{25.5} & {70.5}
            \end{tabular}
            }
            }
            \vspace{-2mm}
            \caption{\textbf{Computation complexity and model parameters.}}
            \label{tab:complexity}
        \end{minipage}
        \quad
        % RealNVP architecture
        \begin{minipage}[t]{0.25\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \makeatletter\def\@captype{table}\makeatother
            \begin{tabular}{c|ccc}        
                ~ & AP & AP$_{50}$ & AP$_{75}$ \\
                \midrule
                $3 \times 64$ & 70.5 & 88.5 & 77.4 \\
                $3 \times 128$ & 70.2 & 88.5 & 77.3 \\
                $3 \times 256$ & 69.6 & 87.9 & 76.5 \\
                $5 \times 32$ & 70.0 & 88.2 & 76.8 \\
                $5 \times 64$ & 70.3 & 88.7 & 77.4 \\
            \end{tabular}
            }
            \vspace{-2mm}
            \caption{\textbf{Different RealNVP Architecture.}}\label{tab:realnvp}
        \end{minipage}
\end{center}
\vspace{-5mm}
\end{table*}
%###########################################################################################

\begin{table}[t]
    \begin{center}
    % \resizebox{\linewidth}{!}{
        \makeatletter\def\@captype{table}\makeatother
        \begin{tabular}{c|ccc}        
            Distribution & AP & AP$_{50}$ & AP$_{75}$ \\
            \midrule
            Const. Var Gaussian ($\ell_2$) & 36.6 & 70.9 & 33.6 \\
            Const. Var Laplace ($\ell_1$) & 58.1 & 82.7 & 65.0 \\
            Gaussian & 60.2 & 82.9 & 66.6 \\
            Laplace & 67.4 & 86.8 & 74.2 \\
            \midrule
            \textbf{RLE ($Q(\bar{\mathbf{x}}) \sim$ Gaussian)} & 70.0 & 88.1 & 76.7 \\
            \textbf{RLE ($Q(\bar{\mathbf{x}}) \sim$ Laplace)} & \textbf{70.5} & \textbf{88.5} & \textbf{77.4} \\
        \end{tabular}
        % }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Initial Density:} Performance with different hypotheses of the output distribution.}\label{tab:density}
    \vspace{-3mm}
\end{table}


\paragraph{Compare with the SOTA on COCO test-dev}
In this experiment, we compare the proposed RLE with the state-of-the-art methods on COCO test-dev. Quantitative results are reported in Tab.~\ref{tab:coco_main}. The proposed regression paradigm significantly outperforms other regression-based methods by \textbf{7.0} mAP and achieves state-of-the-art performance. Compared to the same backbone heatmap-based methods, our regression method is \textbf{1.4} mAP higher with ResNet-152 and \textbf{0.2} mAP higher with HRNet-W48. We demonstrate that heatmap is not the only solution to human pose estimation. Regression-based methods have great potential and can achieve superior performance than heatmap-based methods.

\paragraph{Correlation with Prediction Correctness.}
The estimated standard deviation $\hat{\boldsymbol{\sigma}}$ establishes the correlation with the prediction correctness. The model will a output larger $\hat{\boldsymbol{\sigma}}$ for a more uncertain result. Therefore, $\hat{\boldsymbol{\sigma}}$ plays the same role as the confidence score in the heatmap. We transform the deviation to confidence with Eq.~\ref{eq:conf}. To analysis the correlation of $\hat{\boldsymbol{\sigma}}$ and the prediction correctness, we calculate the Pearson correlation coefficient between the confidence and the OKS to the ground truth on the COCO validation set. The confidence of the heatmap-based prediction~\cite{xiao2018simple} is the maximum value of the heatmap. Tab.~\ref{tab:corr} reveals that RLE has much a stronger correlation to OKS than the heatmap-based method (\textbf{15.2}\% improvement). In real-world applications and other downstream tasks, a reliable confidence score is useful and necessary. RLE address the lack of confidence scores in regression-based methods and provide a more reliable score than the heatmap-based methods.


\paragraph{Computation Complexity.}
The experimental results of computation complexity and model parameters are listed in Tab.~\ref{tab:complexity}. The proposed method achieves comparable results to the heatmap-based methods with significantly lower computation complexity and fewer model parameters. Specifically, the total FLOPs are reduced by \textbf{58.8}\%, and the parameters are reduced by \textbf{30.6}\%. We further calculate the FLOPs of the network head to remove the influence of the network backbone. It shows that the FLOPs of the regression head is only \textbf{1/28500} of the heatmap head, which is almost negligible. The computational superiority of our proposed regression paradigm is of great value in the industry.

\subsection{Ablation Study}

\paragraph{RealNVP Architecture.} In Tab.~\ref{tab:realnvp}, we compare different network architecture of the RealNVP~\cite{dinh2016density} model. It shows that the final AP keeps stable with different RealNVP architecture. We argue that learning the residual log-likelihood is easy for the flow model. Thus the results are robust to the change of the architecture.

\paragraph{Initial Density.} To examine how the assumption of the output distribution affects the regression performance in the context of MLE, we compare the results of different density functions with our method. The Laplace distribution and Gaussian distribution will degenerate to standard $\ell_1$ and $\ell_2$ loss if they are assumed to have constant variances. As shown in Tab.~\ref{tab:density}, the learned distributions of our method provide more than 21.3\% improvements. Different initial densities $Q(\bar{\mathbf{x}})$ for RLE are also tested. There is a large gap between the Gaussian distribution and the Laplace distribution. However, with RLE to learn the change of the density, the difference between these two distributions is significantly reduced. It demonstrates that RLE is robust to different assumptions of the initial density.

% It is seen that the Laplace distribution provide consistent improvements over the Gaussian distribution. \textcolor{red}{[refine]}

% \begin{table}[t]
%     \begin{center}
%     \resizebox{\linewidth}{!}
%     {%
%         \begin{tabular}{l|cccc}
%             Model & \#Params & GFLOPs & AP \\
%             \midrule
%             SimplePose~\cite{xiao2018simple} & 34.0 & 12.9 & 70.9 \\
%             Integral~\cite{integral} & & & 63.4\\
%             \midrule
%             SimpleRLE (Ours) & \textbf{23.6} & \textbf{5.4} & \textcolor{red}{70.5}
%         \end{tabular}
%     }
%     \end{center}
%     \caption{\textbf{Computation complexity and model parameters.}}
%     \label{tab:complexity}
% \end{table}


% \paragraph{Convergence}

% \subsection{Compare with the State-of-the-art}
% In this experiment, we compare the proposed RLE with the state-of-the-art methods on COCO test-dev. Quantitative results are reported in Tab.~\ref{tab:coco_main}. The proposed regression paradigm significantly outperforms other regression-based methods by \textbf{7.0} mAP and achieves state-of-the-art performance. Compared to the same backbone heatmap-based methods, our regression method is \textbf{1.4} mAP higher with ResNet-152 and \textbf{0.2} mAP higher with HRNet-W48. We demonstrate that heatmap is not the only solution to human pose estimation. Regression-based methods have great potential and can achieve superior performance than heatmap-based methods.

% \begin{figure}[t]
%     \begin{center}
%     \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%     %\includegraphics[width=0.8\linewidth]{egfigure.eps}
%     \end{center}
%     \caption{\textbf{Convergence curve.}}
%     \label{fig:convergence}
% \end{figure}

% \begin{table}[t]
%     \begin{center}
%     \resizebox{\linewidth}{!}
%     {%
%         \begin{tabular}{l|ccccccc|c}
%             Method & Hea & Sho & Elb & Wri & Hip & Kne & Ank & Total \\
%             \midrule
%             \textit{heatmap-Based} \\
%             Insafutdinov \etal~\cite{} & 96.8 & 95.2 & 89.3 & 84.4 & 88.4 & 83.4 & 78.0 & 88.5 \\
%             Wei \etal~\cite{} & 97.8 & 95.0 & 88.7 & 84.0 & 88.4 & 82.8 & 79.4 & 88.5 \\
%             Bulat \etal~\cite{} & 97.9 & 95.1 & 89.9 & 85.3 & 89.4 & 85.7 & 81.7 & 89.7 \\
%             Newell \etal~\cite{} & 98.2 & 96.3 & 91.2 & 87.1 & 90.1 & 87.4 & 83.6 & 90.9 \\
%             Sun \etal~\cite{}  & 98.1 & 96.2 & 91.2 & 87.2 & 89.8 & 87.4 & 84.1 & 91.0 \\
%             Tang \etal~\cite{}  & 97.4 & 96.4 & 92.1 & 87.7 & 90.2 & 87.7 & 84.3 & 91.2 \\
%             Ning \etal~\cite{}  & 98.1 & 96.3 & 92.2 & 87.8 & 90.6 & 87.6 & 82.7 & 91.2 \\
%             Luvizon \etal~\cite{} & 98.1 & 96.6 & 92.0 & 87.5 & 90.6 & 88.0 & 82.7 & 91.2 \\
%             Chu \etal~\cite{} & 98.5 & 96.3 & 91.9 & 88.1 & 90.6 & 88.0 & 85.0 & 91.5 \\
%             Chou \etal~\cite{} & 98.2 & 96.8 & 92.2 & 88.0 & 91.3 & 89.1 & 84.9 & 91.8 \\
%             Chen \etal~\cite{} & 98.1 & 96.5 & 92.5 & 88.5 & 90.2 & \textbf{89.6} & 86.0 & 91.9 \\
%             Yang \etal~\cite{} & 98.5 & 96.7 & 92.5 & 88.7 & 91.1 & 88.6 & 86.0 & 92.0 \\  
%             Ke \etal~\cite{} & 98.5 & 96.8 & 92.7 & 88.4 & 90.6 & 89.3 & \textbf{86.3} & 92.1 \\  
%             Tang \etal~\cite{} & 98.4 & \textbf{96.9} & 92.6 & 88.7 & \textbf{91.8} & 89.4 & 86.2 & \textbf{92.3} \\ 
%             SimpleBaseline~\cite{}& 98.5 & 96.6 & 91.9 & 87.6 & 91.1 & 88.1 & 84.1 & 91.5 \\
%             HRNet-W32~\cite{} &\textbf{98.6}  & \textbf{96.9}  & \textbf{92.8}  & \textbf{89.0}  & 91.5  & 89.0 & 85.7 & \textbf{92.3} \\
%             \midrule
%             \textit{Regression Based} \\
%             Carreira \etal~\cite{} \\
%             Sun \etal~\cite{} \\
%             Integral~\cite{integral} \\
%             \textbf{SimpleRLE (ResNet-50)} \\
%             \textbf{SimpleRLE (HRNet-W32)}
%         \end{tabular}
%     }
%     \end{center}
%     \caption{\textbf{Results on MPII test set (PCKh@0.5).}}
%     \label{tab:mpii_main}
% \end{table}


\section{Experiments on MPII}\label{sec:exp_mpii}

In multi-person pose estimation, the final mAP is affected by both the location accuracy and the confidence score. To study how RLE affect the location accuracy and eliminate the impact of the confidence score, we evaluate the proposed regression paradigm on the MPII~\cite{mpii} dataset. Following previous settings~\cite{integral}, PCK and AUC are used for evaluation. We adopt the same ResNet-50 + FC model for single-person 2D pose estimation. Data augmentations and training settings are similar to the experiments on COCO.
% MPII is the benchmark dataset for single-person 2D pose estimation. In total, there are about 29k annotated poses for training and 7k for testing.
% \paragraph{Implementation Details}
% The input image is resized to $256 \times 192$. Data augmentation includes random scale ($\pm 25\%$), rotation ($\pm 45^\circ$), flip and random half-body croping. The learning rate is set to $1 \times 10^{-3}$ at first and reduced by a factor of $10$ at the $170$th and $200$th epoch. We use the Adam solver and train for $210$ epochs, with a mini-batch size of $32$ per GPU and $8$ GPUs in total.
%The testing procedure is almost the same to that in COCO except that we adopt the standard testing strategy to use the provided person boxes instead of detected person boxes. Following ~\cite{}, a six-scale pyramid testing procedure is performed.

\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
        \begin{tabular}{c|ccc}
            Method & PCKh@0.5 & PCKh@0.1 & AUC \\
            \midrule
            Direct Regression & 83.8 & 23.6 & 52.6 \\
            SimplePose (Heatmap)~\cite{xiao2018simple} & \textbf{87.1} & {25.4} & \textbf{56.2} \\
            % Integral Pose~\cite{integral} & 86.5 & 31.0 & 57.8 \\
            \midrule
            \textbf{Regression with RLE} & 85.5 & {26.7} & 55.1 \\
            *\textbf{Regression with RLE} & 85.8 & \textbf{27.1} & 55.5 \\
            % \textbf{Integral + RLE} & 86.9 & \textbf{33.3} & \textbf{59.0}
        \end{tabular}
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Effect of Residual Log-likelihood Estimation on MPII validation set.}}
    \label{tab:ablation_mpii}
    \vspace{-3mm}
\end{table}

\paragraph{Ablation Study.}
Tab.~\ref{tab:ablation_mpii} shows the comparison among methods using heatmaps, direct regression and RLE. RLE surpasses the direct regression baseline. While MPII is less challenging than COCO, the improvement is still significant on PCKh@0.1 (\textbf{13.1}\%) with high localization accuracy requirement. Compared to the heatmap-based method, RLE achieves comparable performance (5.1\% PCKh@0.1 higher, 1.8\% PCKh@0.5 lower and 1.9\% AUC lower), and the pre-trained model achieves the best PCKh@0.1 results. RLE shows the superiority in high precision localization.
% Besides, the combination of integral regression and RLE shows the most accurate localization ability. It outperforms the heatmap based method on PCKh@0.1 by \textbf{10.3}\%, revealing the effectiveness and flexibility of our proposed regression paradigm.
% Tab.~\ref{tab:ablation_mpii} shows the PCKh@0.5 results. We implementation the SimpleRLE model with two model backbone, ResNet-50 and HRNet-W32. Our models are trained on MPII data, no extra data is added. It is shown that the proposed method outperform other regression-based methods and achieves competitive results with the heatmap-based methods. \textcolor{red}{[more]}


%###########################################################################################
% \begin{table*}[t]
%     \begin{center}
%         \begin{minipage}[t]{0.49\textwidth}
%             \centering
%             \resizebox{\linewidth}{!}
%             {%
%             \begin{tabular}{l|cccccc|c}
%                 Method & \tabincell{c}{Zhou \\ \cite{}} & \tabincell{c}{Martinez \\ \cite{}} & \tabincell{c}{Fang \\ \cite{}} & \tabincell{c}{Sun \\ \cite{}} & \tabincell{c}{Sun \\ \cite{}} & \tabincell{c}{Moon \\ \cite{}} & SimpleRLE (Ours) \\
%                     \midrule
%                     MPJPE & & & & & & & \textbf{48.8}
%                 \end{tabular}
%             }
%             \caption{\textbf{Results on Human3.6M.} (Single-stage)}
%             \label{tab:h36m_single_main}
%         \end{minipage}
%         ~
%         \begin{minipage}[t]{0.49\textwidth}
%             \centering
%             \resizebox{\linewidth}{!}
%             {%
%                 \begin{tabular}{l|cccccc|c}
%                     Method & \tabincell{c}{Zhou \\ \cite{}} & \tabincell{c}{Martinez \\ \cite{}} & \tabincell{c}{Fang \\ \cite{}} & \tabincell{c}{Sun \\ \cite{}} & \tabincell{c}{Sun \\ \cite{}} & \tabincell{c}{SRNet \\ \cite{}} & SRNet + RLE (Ours) \\
%                     \midrule
%                     MPJPE
%                 \end{tabular}
%             }
%             \caption{\textbf{Results on Human3.6M.} (Two-stage)}
%             \label{tab:h36m_two_main}
%         \end{minipage}
%     \end{center}
% \end{table*}
%###########################################################################################


\section{Experiments on Human3.6M}\label{sec:exp_h36m}

Human3.6M~\cite{h36m} is an indoor benchmark for 3D pose estimation. For evaluation, MPJPE and PA-MPJPE are used. Following typical protocols~\cite{integral}, we use (S1, S5, S6, S7, S8) for training and (S9, S11) for evaluation.
% It includes 11 subjects (5 females and 6 males) performing 15 different activities in a laboratory environment

\paragraph{Implementation Details.}
% There are two types of approaches to the problem of single-person 3D pose estimation: \textit{single-stage} and \textit{two-stage}.
% The FC layer consists of $K \times 4$ neurons.

For the \textit{single-stage} approach, we adopt the same ResNet-50 + FC architecture. The input image is resized to $256 \times 256$. Data augmentation includes random scale ($\pm 30\%$), rotation ($\pm 30^\circ$), color ($\pm 20\%$) and flip. The learning rate is set to $1 \times 10^{-3}$ at first and reduced by a factor of $10$ at the $90$th and $120$ epoch. We use the Adam solver and train for $140$ epochs, with a mini-batch size of $32$ per GPU and $8$ GPUs in total. The 2D and 3D mixed data training strategy (MPII + Human3.6M) is applied. The testing procedure is the same as the previous works~\cite{integral}.

For the \textit{two-stage} approach, we embed the proposed regression paradigm into the classic baseline~\cite{martinez2017simple} and the state-of-the-art model~\cite{zeng2020srnet}. 2D ground-truth poses are taken as inputs. For data normalization, we follow previous works~\cite{zeng2020srnet,pavllo2019videopose3d,zhaoCVPR19semantic}. Horizontal flip is used during training and inference. The initial learning rate is $1 \times 10^{-3}$ and decays $5\%$ after each epoch. We use the Adam solver and train for $80$ epochs, with a mini-batch size of $1024$.
% to normalize 2d pose into $[-1,1]$ according to the width and height of images, and normalize 3d pose under camera coordinate system to a relative coordinate, which takes the root keypoint as the origin.
% For model structure, we compare six-layer structure with other methods. Each layer, except the output layer, is consist of batch normalization, LeakyReLU. And every two layers are connected by a residual connection. The dimension of hidden layers is $1024$.
% For data augmentation, like ~\cite{pavllo2019videopose3d,zeng2020srnet}, we use horizontal flip during training and inference stages.
% Furthermore, we also use Adam as the optimizer and train $80$ epochs from scratch. The batch size is $1024$.



\paragraph{Ablation Study.} In Tab.~\ref{tab:ablation_h36m}, we report the performance comparison between RLE and the baselines on both \textit{single-stage} and \textit{two-stage} approaches. It is seen that RLE reduces the error of \textit{single-stage} regression baseline by \textbf{1.5} mm and the heatmap-based Integral Pose~\cite{integral} by \textbf{0.6} mm. Besides, without 3D heatmaps, our regression method significantly reduces the FLOPs by \textbf{61.7}\% and the model parameters by \textbf{30.6}\%. For the \textit{two-stage} approach, RLE brings \textbf{2.7} mm improvement to the regression baseline without any test-time overhead.

\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
        \begin{tabular}{l|cc|cc}
            Method & \#Params & GFLOPs & MPJPE~$\downarrow$ & PA-MPJPE~$\downarrow$ \\
            \midrule
            \multicolumn{2}{l}{\textit{Single-stage}} \\
            Direct Regression & 23.8M & 5.4 & 50.1 & 39.3 \\
            Integral Pose~\cite{integral} & 34.3M & 14.1 & 49.2 & 39.1 \\
            \textbf{Regression with RLE} & \textbf{23.8M} & \textbf{5.4} & \textbf{48.6} & \textbf{38.5} \\
            % \textbf{Integral + SimpleRLE} & & {48.9} \\
            \midrule
            \multicolumn{2}{l}{\textit{Two-stage}} \\
            FC Baseline & 4.3M & 0.275 & 43.6 & 33.2 \\
            \textbf{FC Baseline + RLE} & 4.3M & 0.275 & \textbf{40.9} & \textbf{31.1}
        \end{tabular}
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Ablation study on Human3.6M.}}
    \label{tab:ablation_h36m}
    \vspace{-1mm}
\end{table}

\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
    \begin{tabular}{l|ccccc|c}
        Method &\tabincell{c}{Sun \\ \cite{sun2017compositional}} & \tabincell{c}{Nibali \\ \cite{nibali20193d}} &  \tabincell{c}{Sun \\ \cite{integral}} & \tabincell{c}{Moon \\ \cite{moon}} & \tabincell{c}{Zhou \\ \cite{zhou2019hemlets}} & Ours \\
            \midrule
            \#Params & - & 57.9M & 34.3M & 34.3M & 49.6M & \textbf{23.8}M \\
            GFLOPs & - & 29.3 & 14.1 & 14.1 & 41.4 & \textbf{5.4} \\
            MPJPE & 59.1 & 49.5 & 49.6 & 53.3 & \textbf{47.7} & 48.6
        \end{tabular}
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Single-stage Results on Human3.6M.}}
    \label{tab:h36m_single_main}
    \vspace{-1mm}
\end{table}

\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
    % \setlength{\tabcolsep}{1mm}{
        \begin{tabular}{l|cccccc|c}
            % Method  & \tabincell{c}{Pose2Mesh \\ \cite{choi2020pose2mesh}} &\tabincell{c}{FC Baseline \\ \cite{martinez2017simple}} & \tabincell{c}{SemGCN \\ \cite{zhaoCVPR19semantic}} & \tabincell{c}{SemGCN \\w/PG \cite{fang2018learning}} & \tabincell{c}{Pre-agg GCN\\ \cite{liu2020comprehensive}} & \tabincell{c}{SRNet \\ \cite{zeng2020srnet}} & \tabincell{c}{SRNet + RLE \\ (Ours)} \\
            Method  & \tabincell{c}{Choi \\ \cite{choi2020pose2mesh}} &\tabincell{c}{Martinez \\ \cite{martinez2017simple}} & \tabincell{c}{Zhao \\ \cite{zhaoCVPR19semantic}} & \tabincell{c}{Fang \\ \cite{fang2018learning}} & \tabincell{c}{Liu\\ \cite{liu2020comprehensive}} & \tabincell{c}{Zeng \\ \cite{zeng2020srnet}} & \tabincell{c}{Ours} \\
            \midrule
            MPJPE & 55.5 & 45.5 & 43.8 & 42.5 & 37.8 & 36.5 & \textbf{36.3} \\
        \end{tabular}
    % }
    }
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Two-stage Results on Human3.6M.} Our result is based on SRNet~\cite{zeng2020srnet} with RLE.}
    \label{tab:h36m_two_main}
    \vspace{-3mm}
\end{table}

\paragraph{Compare the the State-of-the-art.}
In this experiment, we compare the proposed regression paradigm with both \textit{single-stage} and \textit{two-stage} state-of-the-art methods in Tab.~\ref{tab:h36m_single_main} and Tab.~\ref{tab:h36m_two_main}. For \textit{single-stage}, our method achieves comparable performance to the state-of-the-art methods while reducing the FLOPs by \textbf{86.7}\%. The model parameters and FLOPs are calculated using the official code of these methods. Note that \cite{zhou2019hemlets} only releases the testing code. For fare comparison, we re-train the model with the same training settings as ours. For \textit{two-stage}, our method is based on SRNet~\cite{zeng2020srnet} with RLE. It achieves state-of-the-art performance by 0.2 mm improvement to the original SRNet.

==> sections/sepool.tex <==
\subsection{Spatial Equivariant Pooling}\label{sec:pooling}

\begin{figure}[t]
    \begin{center}
    \fbox{\rule{0pt}{2.5in} \rule{0.9\linewidth}{0pt}}
    %\includegraphics[width=0.8\linewidth]{egfigure.eps}
    \end{center}
    \caption{Illustrasion of spatial translation equivariance.}
    \label{fig:equivarance}
\end{figure}

Detection based approaches utilize a likelihood heat map for each joint to indicate the its occurrence probability. This privileged form of representation fits with a characteristics of the convolution operation, named \textit{spatial translation equivariance}~\cite{}. It contributes to the recent performance leaps of human pose estimation.
%This characteristics is \textit{spatial translation equivariance}.
As shown in Fig.~\ref{fig:equivarance}, when the input is translated, the output of the convolutional layer should be transformed accordingly. The spatial translation equivariance can be formulated as:
\begin{equation}
    \textit{Conv}(T_{\Delta x}(h)) = T_{\Delta x}(\textit{Conv}(h)),
\end{equation}
where $h$ denotes the input features, $\Delta x$ denotes the displacement, $T_{\Delta x}(\cdot)$ denotes the translation operation based on $\Delta x$ and $\textit{Conv}(\cdot)$ denotes the convolution operation. The modern fully convolutional models like ResNet~\cite{resnet}, Hourglass~\cite{newell2016stacked}, HRNet~\cite{sun2019deep} contain some operations that make the model not perfectly translation equivarant, \eg down-sampling and max-pooling. Still, it is easy for these models to learn this characteristics.

In contrast, it is hard for the conventional regression based approach to learn the translation equivarance. Assuming that $h$ is the output features of the CNN model, $h \in \mathbb{R}^{C \times H \times W}$, where $C$ is the number of feature channels, $H$ is the height and $W$ is the width. An average pooling layer is used to squeeze the features and a subsequent fully connected layer is used to regress the coordinates. This process is denoted as:
\begin{equation}
    \hat{x} = \langle \mathbf{w}, \textit{avg}(h) \rangle,
    \label{eq:avg}
\end{equation}
where $\hat{x}$ is the predicted coordinate, $\mathbf{w}$ is the weight of the fully connected layer and $\langle\cdot,\cdot\rangle$ denotes a dot product. For simplicity, we take 1-dimensional features as an example, \ie $W = 1$, and $\mathbf{h}_i \in \mathbb{R}^C$ denotes the $i$-th feature. Eq.~\ref{eq:avg} can be re-formulated as:
\begin{equation}
    \hat{x} = \langle \mathbf{w}, \frac{1}{H} \sum_{i} \mathbf{h}_i \rangle.
\end{equation}
If the translation equivarance holds, the regression output should be transformed accordingly to the translated input features $T_{\Delta x}(h)$, \ie $T_{\Delta x}(\hat{x}) = \hat{x} + \Delta x$. We denote $\tilde{h} = T_{\Delta x}(h)$, where $\tilde{\mathbf{h}}_i = \mathbf{h}_{i - \Delta x}$. Since the sum of the features won't be affected by the translation, it is easy to demonstrate that the conventional regression paradigm is invariant to translation:
{\small
\begin{equation}
    \begin{aligned}
    \langle\mathbf{w}, \textit{avg}(T_{\Delta x}(h)) \rangle &= \langle \mathbf{w}, \frac{1}{H} \sum_{i} \tilde{\mathbf{h}}_i \rangle
    = \langle \mathbf{w}, \frac{1}{H} \sum_{i} \mathbf{h}_i \rangle \\
    &= \hat{x} \not= T_{\Delta x}(\hat{x}) = T_{\Delta x}(\langle \mathbf{w}, \textit{avg}(h) \rangle) ,
    \end{aligned}
\end{equation}
}where $\sum_i \mathbf{h}_i = \sum_i \mathbf{h}_{i - \Delta x} = \sum_i \tilde{\mathbf{h}}_i$. Therefore, the CNN models have to learn a more complicated mapping function to encode the spatial information, which increases the difficulty of learning and reduces the generalization ability.

To tackle this problem, we develop a simple yet effective method named Spatial Equivariant Pooling (SEPooling), to facilitate the spatial information learning. The process of SEPooling is formulated as:
\begin{equation}
    \textit{SEPool}(h) = \frac{1}{H} \sum_{i} i \cdot \mathbf{h}_i.
\end{equation}
The regression process using SEPooling with a translated input feature can be formulated as:
{\small
\begin{equation}
    \begin{aligned}
        &\langle \mathbf{w}, \textit{SEPool}(T_{\Delta x}(h)) \rangle \\
        = &\langle \mathbf{w}, \frac{1}{H} \sum_{i} i \cdot \tilde{\mathbf{h}}_i \rangle = \langle \mathbf{w}, \frac{1}{H} \sum_{i} i \cdot {\mathbf{h}}_{i - \Delta x} \rangle \\
        = &\langle \mathbf{w}, \frac{1}{H} \sum_{i} (i - \Delta x) \cdot {\mathbf{h}}_{i - \Delta x} + \frac{1}{H} \sum_{i} \Delta x \cdot {\mathbf{h}}_{i - \Delta x} \rangle \\
        = &\langle \mathbf{w}, \frac{1}{H} \sum_{i} i \cdot {\mathbf{h}}_{i} \rangle + \Delta x \cdot \langle \mathbf{w}, \frac{1}{H} \sum_{i} {\mathbf{h}}_{i - \Delta x} \rangle \\
        = &~ \hat{x} + \Delta x \cdot \langle \mathbf{w}, \bar{\mathbf{h}} \rangle,
    \end{aligned}
\end{equation}
}where $\bar{\mathbf{h}}$ denotes the average value of all $\mathbf{h}_i$. In order for the output to be transformed according to the input feature, we only need to add a regularization term to make sure $\langle \mathbf{w}, \bar{\mathbf{h}} \rangle = 1$, \ie $\mathcal{L}_{\textit{reg}} = \| \langle \mathbf{w}, \bar{\mathbf{h}} \rangle - 1 \|_1$. In this way, the condition of equivarance can be maintained:
\begin{equation}
    \begin{aligned}
        \langle \mathbf{w}, \textit{SEPool}(T_{\Delta x}(h)) \rangle &= \hat{x} + \Delta x = T_{\Delta x}(\hat{x})\\
        &= T_{\Delta x}(\langle \mathbf{w}, \textit{SEPool}(h) \rangle).
    \end{aligned}
\end{equation}

With the proposed SEPooling operation, we observe that the regression model converge faster while training and obtain better performance. 
%When the translation operation $T_{\Delta x}(\cdot)$ is applied to $h$, we obtain $\tilde{h} = T_{\Delta x}(h)$, where $\tilde{\mathbf{h}}_i = \mathbf{h}_{i - \Delta x}$.




==> supp_sections/ablation_study_new.tex <==
\section{More Ablation Experiments}\label{sec:ablation}


\begin{table}[t]
    \begin{center}
    \resizebox{\linewidth}{!}
    {%
        \setlength{\tabcolsep}{1.2mm}{
        \begin{tabular}{c|ccc|cc}
            \multirow{2}{*}{Method} & \multicolumn{3}{c|}{MPII} & \multicolumn{2}{c}{Human3.6M} \\
            \cmidrule(lr){2-4} \cmidrule(lr){5-6}
            & PCKh@0.5 & PCKh@0.1 & AUC & MPJPE & PA-MPJPE\\
            \midrule
            % Integral Pose~\cite{integral} & 86.5 & 31.0 & 57.8 \\
            % Direct Regression & 83.8 & 23.6 & 52.6 \\
            \textbf{DLE} & 84.3 & 25.3 & 53.5 & - & - \\
            \textbf{RLE} & \textbf{85.5} & \textbf{26.7} & \textbf{55.1} & \textbf{48.6} & \textbf{38.5} \\
            % *\textbf{Regression with RLE} & 85.8 & \textbf{27.1} & 55.5 \\
            % \textbf{Integral + RLE} & 86.9 & \textbf{33.3} & \textbf{59.0}
        \end{tabular}
        }
    }
    \end{center}
    \caption{\textbf{Comparison between DLE and RLE} on MPII and Human3.6M.}
    \label{tab:dle}
\end{table}

\paragraph{Comparison between DLE and RLE}
In this work, direct likelihood estimation (DLE) refers to the model that only adopts the reparameterization strategy to estimate the likelihood function. The comparison is conducted on COCO~\cite{mscoco} validation set in the paper. Here, we provide more comparison results on MPII~\cite{mpii} and Human3.6M~\cite{h36m} datasets, listed in Tab.~\ref{tab:dle}. It is seen that RLE shows consistent improvements over DLE.

\begin{table}[t]
    \begin{center}
        \resizebox{\linewidth}{!}
        {
            \begin{tabular}{c|c|c|c}
                Method & reg. loss weight & hm. loss weight & AP \\
                \midrule
                Direct Regression ($\ell_1$) & 1 & 1 & 57.5 \\
                Direct Regression ($\ell_1$) & 1 & 0.5 & 56.7 \\
                Direct Regression ($\ell_1$) & 1 & 0 & 58.1 \\
                \midrule
                RLE & 1 & 1 & 70.4 \\
                RLE & 1 & 0.5 & 70.2 \\
                RLE & 1 & 0 & 70.5 \\

            \end{tabular}
        }
    \end{center}
    \caption{\textbf{Effect of the auxiliary heatmap loss.}}
    \label{tab:aux}
\end{table}

\paragraph{Auxiliary Heatmap Loss}
In this experiment, we add an auxiliary heatmap loss to the regression model and study its effect. The regression models follow the top-down framework with the ``ResNet-50 + FC'' architecture. To train the model with the auxiliary loss, the ResNet-50 backbone is followed by 3 deconv layers as SimplePose~\cite{xiao2018simple} to generate heatmaps. The deconv layers are parallel to the FC layer. Thus the model can predict both heatmaps and the regressed coordinates. Further, we study the effectiveness of combining the auxiliary loss and the heatmap pre-trained backbone. Quantitative results are shown in Tab.~\ref{tab:aux} and Tab.~\ref{tab:baseline}. 

\begin{table}[t]
    \begin{center}
        \resizebox{\linewidth}{!}
        {
            \begin{tabular}{c|c|c|c}
                Method & hm. loss & hm. pretrained & AP \\
                \midrule
                Direct Regression ($\ell_1$) & $\times$ & $\times$ & 58.1 \\
                Direct Regression ($\ell_1$) & \checkmark & $\times$ & 57.5 \\
                Direct Regression ($\ell_1$) & $\times$ & \checkmark & \\
                Direct Regression ($\ell_1$) & \checkmark & \checkmark & \\
                \midrule
                Laplace Regression & $\times$ & $\times$ & 67.4 \\
                Laplace Regression & \checkmark & $\times$ & \\
                Laplace Regression & $\times$ & \checkmark & \\
                Laplace Regression & \checkmark & \checkmark & \\
                \midrule
                RLE & $\times$ & $\times$ & 70.5 \\
                RLE & \checkmark & $\times$ & \\
                RLE & $\times$ & \checkmark & 71.3 \\
                RLE & \checkmark & \checkmark & \\
            \end{tabular}
        }
    \end{center}
    \caption{\textbf{Effect of heatmap pre-trained backbone and auxiliary heatmap loss.}}
    \label{tab:baseline}
\end{table}

% \paragraph{Comparison with More Regression Baseline.}

==> supp_sections/curve.tex <==
\section{Training Curves}\label{sec:curve}
